Towards Probabilistic Verification of Machine Unlearning

The right to be forgotten, also known as the right to erasure, is the right of individuals to have their data erased from an entity storing it. The status of this long held notion was legally solidified recently by the General Data Protection Regulation (GDPR) in the European Union. Consequently, there is a need for mechanisms whereby users can verify if service providers comply with their deletion requests. In this work, we take the first step in proposing a formal framework to study the design of such verification mechanisms for data deletion requests -- also known as machine unlearning -- in the context of systems that provide machine learning as a service (MLaaS). Our framework allows the rigorous quantification of any verification mechanism based on standard hypothesis testing. Furthermore, we propose a novel backdoor-based verification mechanism and demonstrate its effectiveness in certifying data deletion with high confidence, thus providing a basis for quantitatively inferring machine unlearning. We evaluate our approach over a range of network architectures such as multi-layer perceptrons (MLP), convolutional neural networks (CNN), residual networks (ResNet), and long short-term memory (LSTM), as well as over 5 different datasets. We demonstrate that our approach has minimal effect on the ML service's accuracy but provides high confidence verification of unlearning. Our proposed mechanism works even if only a handful of users employ our system to ascertain compliance with data deletion requests. In particular, with just 5% of users participating, modifying half their data with a backdoor, and with merely 30 test queries, our verification mechanism has both false positive and false negative ratios below $10^{-3}$. We also show the effectiveness of our approach by testing it against an adaptive adversary that uses a state-of-the-art backdoor defense method.

==> Images/experiment_results/text_files/AGNews_natural.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/agnews_lstm_natural_acc.png}
		\caption{Accuracy performance for AG News classifiers with varied poison ratio}
		\label{fig:nat_agnews_acc}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/experiment_results/agnews_lstm_natural_verify_a_1e-5.png}
		\caption{Verification performance for AG News classifiers with different poison ratios. We fix the $\alpha$ to be $10^{-5}$.}
		\label{fig:nat_agnews_verify_ratio}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/agnews_lstm_natural_verify_position_ratio_30.png}
		\caption{Verification performance with different numbers of test samples for the AG News classifier with poison ratio of $30\%$.}
		\label{fig:nat_agnews_verify_alpha}
	\end{subfigure}\hfill
	\caption{Performance for AG News dataset.
	}
	\label{fig:nat_agnews}
\end{figure*}

==> Images/experiment_results/text_files/CIFAR_defended.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/CIFAR_resnet_defended_acc.png}
		\caption{Accuracy performance for CIFAR10 classifiers with varied poison ratio}
		\label{fig:def_cifar_acc}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/experiment_results/CIFAR_resnet_defended_verify_a_1e-5.png}
		\caption{Verification performance for CIFAR10 classifiers with different poison ratios. We fix the $\alpha$ to be $10^{-5}$.}
		\label{fig:def_cifar_verify_ratio}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/CIFAR_resnet_defended_verify_position_ratio_30.png}
		\caption{Verification performance with different numbers of test samples for the CIFAR10 classifier with poison ratio of $30\%$.}
		\label{fig:def_cifar_verify_alpha}
	\end{subfigure}\hfill
	\caption{Performance for CIFAR10 dataset with backdoor defense.
	}
	\label{fig:def_cifar}
\end{figure*}

==> Images/experiment_results/text_files/CIFAR_natural.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/CIFAR_resnet_natural_acc.png}
		\caption{Accuracy performance for CIFAR10 classifiers with varied poison ratio}
		\label{fig:nat_cifar_acc}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/experiment_results/CIFAR_resnet_natural_verify_a_1e-5.png}
		\caption{Verification performance for CIFAR10 classifiers with different poison ratios. We fix the $\alpha$ to be $10^{-5}$.}
		\label{fig:nat_cifar_verify_ratio}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/CIFAR_resnet_natural_verify_position_ratio_30.png}
		\caption{Verification performance with different numbers of test samples for the CIFAR10 classifier with poison ratio of 20\%.}
		\label{fig:nat_cifar_verify_alpha}
	\end{subfigure}\hfill
	\caption{Performance for CIFAR10 dataset.
	}
	\label{fig:nat_cifar}
\end{figure*}

==> Images/experiment_results/text_files/EMNIST_defended.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/EMNIST_MLP_defended_acc.png}
		\caption{Accuracy performance for EMNIST classifiers with varied poison ratio}
		\label{fig:def_emnist_acc}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/experiment_results/EMNIST_MLP_defended_verify_a_1e-5.png}
		\caption{Verification performance for EMNIST classifiers with different poison ratios. We fix the $\alpha$ to be $10^{-5}$.}
		\label{fig:def_emnist_verify_ratio}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/EMNIST_MLP_defended_verify_position_ratio_30.png}
		\caption{Verification performance with different numbers of test samples for the EMNIST classifier with poison ratio of $30\%$.}
		\label{fig:def_emnist_verify_alpha}
	\end{subfigure}\hfill
	\caption{Performance for EMNIST dataset with backdoor defense.
	}
	\label{fig:def_emnist}
\end{figure*}

==> Images/experiment_results/text_files/EMNIST_natural.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/EMNIST_MLP_natural_acc.png}
		\caption{Accuracy performance for EMNIST classifiers with varied poison ratio}
		\label{fig:nat_emnist_acc}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/experiment_results/EMNIST_MLP_natural_verify_a_1e-5.png}
		\caption{Verification performance for EMNIST classifiers with different poison ratios. We fix the $\alpha$ to be $10^{-5}$.}
		\label{fig:nat_emnist_verify_ratio}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/EMNIST_MLP_natural_verify_position_ratio_30.png}
		\caption{Verification performance with different numbers of test samples for the EMNIST classifier with poison ratio of $30\%$.}
		\label{fig:nat_emnist_verify_alpha}
	\end{subfigure}\hfill
	\caption{Performance for EMNIST dataset.
	}
	\label{fig:nat_emnist}
\end{figure*}

==> Images/experiment_results/text_files/FEMNIST_defended.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/FEMNIST_CNN_defended_acc.png}
		\caption{Accuracy performance for FEMNIST classifiers with varied poison ratio}
		\label{fig:def_femnist_acc}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/experiment_results/FEMNIST_CNN_defended_verify_a_1e-5.png}
		\caption{Verification performance for FEMNIST classifiers with different poison ratios. We fix the $\alpha$ to be $10^{-5}$.}
		\label{fig:def_femnist_verify_ratio}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/FEMNIST_CNN_defended_verify_position_ratio_30.png}
		\caption{Verification performance with different numbers of test samples for the FEMNIST classifier with poison ratio of $30\%$.}
		\label{fig:def_femnist_verify_alpha}
	\end{subfigure}\hfill
	\caption{Performance for FEMNIST dataset with backdoor defense.
	}
	\label{fig:def_femnist}
\end{figure*}

==> Images/experiment_results/text_files/FEMNIST_natural.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/FEMNIST_CNN_natural_acc.png}
		\caption{Accuracy performance for FEMNIST classifiers with varied poison ratio}
		\label{fig:nat_femnist_acc}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\centering
		\includegraphics[width=\linewidth]{Images/experiment_results/FEMNIST_CNN_natural_verify_a_1e-5.png}
		\caption{Verification performance for FEMNIST classifiers with different poison ratios. We fix the $\alpha$ to be $10^{-5}$.}
		\label{fig:nat_femnist_verify_ratio}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/FEMNIST_CNN_natural_verify_position_ratio_30.png}
		\caption{Verification performance with different numbers of test samples for the FEMNIST classifier with poison ratio of $30\%$.}
		\label{fig:nat_femnist_verify_alpha}
	\end{subfigure}\hfill
	\caption{Performance for FEMNIST dataset.
	}
	\label{fig:nat_femnist}
\end{figure*}

==> Images/experiment_results/text_files/defended_model_beta_cdf.tex <==
% \begin{figure*}[!ht]
% 	\centering
% 	\begin{subfigure}[t]{0.32\linewidth}
% 		\raggedleft
% 		\includegraphics[width=\linewidth]{Images/experiment_results/EMNIST_MLP_defended_beta_cdf_poison_ratio_30_alpha_1e-3_10_samples_mini_of_users.png}
% 		\caption{The cumulative distributions of Type-II error with 10 samples on the EMNIST classifier with neural cleanse backdoor defense and poison ratio of $30\%$, we set $\alpha = 10^{-3}$.}
% 		\label{fig:def_emnist_beta_cdf}
% 	\end{subfigure}\hfill
% 	\begin{subfigure}[t]{0.32\linewidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{Images/experiment_results/FEMNIST_CNN_defended_beta_cdf_poison_ratio_30_alpha_1e-3_10_samples_mini_of_users.png}
% 		\caption{The cumulative distributions of Type-II error with 10 samples on the FEMNIST classifier with neural cleanse backdoor defense and poison ratio of $30\%$, we set $\alpha = 10^{-3}$.}
% 		\label{fig:def_femnist_beta_cdf}
% 	\end{subfigure}\hfill
% 	\begin{subfigure}[t]{0.32\linewidth}
% 		\raggedright
% 		\includegraphics[width=\linewidth]{Images/experiment_results/CIFAR_resnet_defended_beta_cdf_poison_ratio_30_alpha_1e-3_10_samples_mini_of_users.png}
% 		\caption{The cumulative distributions of Type-II error with 10 samples on the CIFAR10 classifier with neural cleanse backdoor defense and poison ratio of $30\%$, we set $\alpha = 10^{-3}$.}
% 		\label{fig:def_cifar_beta_cdf}
% 	\end{subfigure}\hfill
% 	\caption{Further analysis into individual users. When obtaining the distributions of $\beta$, we can either choose to use the average $p$ among all undeleted users with different individual deleted user's $q$ value, or revese.
% 	}
% 	\label{fig:def_model_beta_cdf}
% \end{figure*}

==> Images/experiment_results/text_files/defended_model_varied_author_poison.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/author_poison/EMNIST_MLP_50_percent_poison_acc_defended.png}
		\caption{EMNIST}
		\label{fig:nat_emnist_varied_f}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/author_poison/FEMNIST_CNN_50_percent_poison_acc_defended.png}
		\caption{FEMNIST}
		\label{fig:nat_femnist_varied_f}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/author_poison/CIFAR10_resnet_50_percent_poison_acc_defended.png}
		\caption{CIFAR10}
		\label{fig:nat_cifar_varied_f}
	\end{subfigure}\hfill
% 	\begin{subfigure}[t]{0.24\linewidth}
% 		\raggedright
% 		\includegraphics[width=\linewidth]{Images/experiment_results/agnews_lstm_natural_acc_cdf_poison_ratio_30.png}
% 		\caption{AG News}
% 		\label{fig:nat_agnews_acc_cdf}
% 	\end{subfigure}\hfill
	\caption{The model accuracy and backdoor attack accuracy for the adaptive server with different author poison ratio values (poison ratio $50\%$).}
	\label{fig:nat_model_acc_cdf}
\end{figure*}




\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.30\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/author_poison/EMNIST_MLP_50_percent_poison_acc_defended.png}
		\caption{EMNIST}
		\label{fig:nat_emnist_varied_f}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.30\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/author_poison/FEMNIST_CNN_50_percent_poison_acc_defended.png}
		\caption{FEMNIST}
		\label{fig:nat_femnist_varied_f}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.30\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/author_poison/CIFAR10_resnet_50_percent_poison_acc_defended.png}
		\caption{CIFAR10}
		\label{fig:nat_cifar_varied_f}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.05\linewidth}
		\begin{flushleft}
            ~~\rotatebox{90}{~~~~~~~~~Non-adaptive}  
        \end{flushleft}
	\end{subfigure}
	\caption{The model accuracy and backdoor attack accuracy for the adaptive server with different author poison ratio values (poison ratio $50\%$).}
	\label{fig:nat_model_acc_cdf}
\end{figure*}

==> Images/experiment_results/text_files/model_capacity.tex <==
\begin{figure}[!b]
	\centering\vspace{-1em}
	\begin{subfigure}[t]{\linewidth}
		\centering
		\includegraphics[width=0.7\linewidth]{Images/experiment_results/EMNIST_model_capacity_acc.png}
		\caption{Backdoor attack accuracy for undeleted users.}
		\label{fig:capacity_acc}
	\end{subfigure}\hfill
	\par\medskip % force a bit of vertical whitespace
	\begin{subfigure}[t]{\linewidth}
		\centering
		\includegraphics[width=0.7\linewidth]{Images/experiment_results/EMNIST_model_capacity_verify_alpha_1e-5_poison_ratio_30.png}
		\caption{Verification performance for EMNIST classifiers. We fix the poison ratio as $30\%$ and $\alpha$ as $10^{-5}$.}
		\label{fig:capacity_verify}
	\end{subfigure}\hfill
	\caption{Performance on EMNIST dataset with two model architectures (MLP and CNN).}
	\label{fig:model_capacity}
\end{figure}

==> Images/experiment_results/text_files/natural_model_beta_cdf.tex <==
% \begin{figure*}[!ht]
% 	\centering
% 	\begin{subfigure}[t]{0.24\linewidth}
% 		\raggedleft
% 		\includegraphics[width=\linewidth]{Images/experiment_results/EMNIST_MLP_natural_beta_cdf_poison_ratio_30_alpha_1e-3_10_samples_mini_of_users.png}
% 		\caption{The cumulative distributions of Type-II error with 10 test samples on the EMNIST classifier with poison ratio of $30\%$, we set $\alpha = 10^{-3}$.}
% 		\label{fig:nat_emnist_beta_cdf}
% 	\end{subfigure}\hfill
% 	\begin{subfigure}[t]{0.24\linewidth}
% 		\raggedleft
% 		\includegraphics[width=\linewidth]{Images/experiment_results/FEMNIST_CNN_natural_beta_cdf_poison_ratio_30_alpha_1e-3_10_samples_mini_of_users.png}
% 		\caption{The cumulative distributions of Type-II error with 10 test samples on the FEMNIST classifier with poison ratio of $30\%$, we set $\alpha = 10^{-3}$.}
% 		\label{fig:nat_femnist_beta_cdf}
% 	\end{subfigure}\hfill
% 	\begin{subfigure}[t]{0.24\linewidth}
% 		\raggedright
% 		\includegraphics[width=\linewidth]{Images/experiment_results/CIFAR_resnet_natural_beta_cdf_poison_ratio_30_alpha_1e-3_10_samples_mini_of_users.png}
% 		\caption{The cumulative distributions of Type-II error with 10 test samples on the CIFAR10 classifier with poison ratio of $30\%$, we set $\alpha = 10^{-3}$.}
% 		\label{fig:nat_cifar_beta_cdf}
% 	\end{subfigure}\hfill
% 	\begin{subfigure}[t]{0.24\linewidth}
% 		\raggedright
% 		\includegraphics[width=\linewidth]{Images/experiment_results/agnews_lstm_natural_beta_cdf_poison_ratio_30_alpha_1e-3_10_samples_mini_of_users.png}
% 		\caption{The cumulative distributions of Type-II error with 10 test samples on the AG News classifier with poison ratio of $30\%$, we set $\alpha = 10^{-3}$.}
% 		\label{fig:nat_agnews_beta_cdf}
% 	\end{subfigure}\hfill
% 	\caption{Further analysis into individual users. When obtaining the distributions of $\beta$, we can either choose to use the average $p$ among all undeleted users with different individual deleted user's $q$ value, or revese.
% 	}
% 	\label{fig:nat_model_beta_cdf}
% \end{figure*}

==> Images/experiment_results/text_files/natural_model_varied_author_poison.tex <==
\begin{figure*}[!ht]
	\centering
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/author_poison/EMNIST_MLP_50_percent_poison_acc.png}
		\caption{EMNIST}
		\label{fig:nat_emnist_varied_f}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedleft
		\includegraphics[width=\linewidth]{Images/experiment_results/author_poison/FEMNIST_CNN_50_percent_poison_acc.png}
		\caption{FEMNIST}
		\label{fig:nat_femnist_varied_f}
	\end{subfigure}\hfill
	\begin{subfigure}[t]{0.32\linewidth}
		\raggedright
		\includegraphics[width=\linewidth]{Images/experiment_results/author_poison/CIFAR10_resnet_50_percent_poison_acc.png}
		\caption{CIFAR10}
		\label{fig:nat_cifar_varied_f}
	\end{subfigure}\hfill
% 	\begin{subfigure}[t]{0.24\linewidth}
% 		\raggedright
% 		\includegraphics[width=\linewidth]{Images/experiment_results/agnews_lstm_natural_acc_cdf_poison_ratio_30.png}
% 		\caption{AG News}
% 		\label{fig:nat_agnews_acc_cdf}
% 	\end{subfigure}\hfill
	\caption{The model accuracy and backdoor attack accuracy for the naive server with different author poison ratio values (poison ratio $50\%$).}
	\label{fig:nat_model_acc_cdf}
\end{figure*}

==> Images/general.tex <==
\begin{figure*}
\centering
\begin{subfigure}[t]{.32\textwidth}
  \raggedleft
  \includegraphics[width=\linewidth]{1}
  \caption{Phase I: Data Collection}
  \label{fig:sharing}
\end{subfigure}\hfill
\begin{subfigure}[t]{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{2}
  \caption{Phase II: Data Deletion}
  \label{fig:delete}
\end{subfigure}\hfill
\begin{subfigure}[t]{.32\textwidth}
  \raggedright
  \includegraphics[width=\linewidth]{3}
  \caption{Phase III: Verification}
  \label{fig:detect}
\end{subfigure}\hfill
\caption{Our system runs in 3 phases -- Phase I where data is collected from the users, Phase II where users request data to be deleted, and Phase III where the users can statistically verify if their data was deleted with high confidence.}
\label{fig:general}
\end{figure*}

==> Sections/analysis.tex <==
\section{Theoretical Analysis}\label{sec:analysis}

\TODO{This is standard hypothesis testing. Connect with Section 3. Add a table with notation. Talk about relaxation.}

\input{Images/binom}

In this section, we theoretically analyze the confidence of our hypothesis test. The confidence, expressed by the metric $\ourmetric{A, \alpha}{s,n}$, is based on a hypothesis test where two cases are compared: $H_0$ -- the data has been deleted, and $H_1$ -- the data has not been deleted. We measure the Type II error $\beta$ which denotes the probability that the server evades detection, i.e., the server behaves malicious but is not caught. Note that this requires we set a level of acceptable Type I error $\alpha$, i.e., the probability that we falsely accuse the server of avoiding deletion. Hence, the metric $\ourmetric{A, \alpha}{s,n} = 1 - \beta$ is a function of the backdoor strategy $s$ and the number of predictions on backdoored test samples $n$ for a given MLaaS server $A$ and a value of Type I error $\alpha$. We structure the section as follows: 

\begin{enumerate}[label=(\Alph*)]
    \item \textbf{Basic Hypothesis Testing:} First we set-up the basics of hypothesis testing for our scenario and introduce the required notation.
    \item \textbf{Estimating Deletion Confidence:} Next, we show how to compute the metric $\ourmetric{A, \alpha}{s,n}$ for a given Type I error $\alpha$. This can be reduced to the following steps:
    \begin{itemize}
        \item Compute the optimal value of the threshold $t$ for a given value of $\alpha$, the Type I error
        \item Compute the value of $\beta$, the Type II error, for the given optimal threshold $t$
        \item Compute $\ourmetric{A, \alpha}{s,n}$ from the previously computed $\beta$
    \end{itemize}
    \item \textbf{Relaxing Assumptions:} 
    %We have assumed the knowledge of some statistics $p$ and $q$ perfectly in the previous computation. This is difficult for single users to estimate and we provide techniques to estimate these as well as bounds on how well these estimates capture the system.
    Our theoretical analysis is based on prior knowledge of statistics defining the hypotheses $H_0$ and $H_1$. Next, we outline strategies for users to estimate these statistics, and theoretically quantify the impact of the estimation on our system.
\end{enumerate}


\subsection{Basic Hypothesis Testing}
We query the ML-mechanism $A$ with $n$ backdoored samples $\{\mathsf{sample_i}\}_{i=1}^n$ of a single user and measure how often the ML-mechanism does classify the samples as the desired target label, denoted as $\mathsf{Target_i}$.
%as opposed to the true label of the sample.
%Let us denote by $\mathsf{True_i}$ and $\mathsf{Target_i}$ the true label and the target label of a sample $\mathsf{sample}_i$. 
Then, the measured success rate is 
%\grey{comment by Liwei: $\hat{m}$ should be average value.}
\begin{equation}
    \hat{r} = \frac{1}{n} \sum_{i=1}^n 
    \begin{cases}
        1 \text{ if } A(\mathsf{sample_i}) = \mathsf{Target_i} \\
        0 \text{ otherwise}
    \end{cases}
\end{equation}

Furthermore, we define two important quantities, $q, p$ that quantify the probability that the prediction on backdoored samples is equal to the target label for the null hypothesis vs the alternative hypothesis. %In other words, let $q, p$ be defined as follows:
\begin{equation}\label{eq:pandq}
\begin{aligned}
  q &= \pr{A(\mathsf{sample_i}) = \mathsf{Target_i} \, | \, H_0 \textrm{ is true}} \\
  p &= \pr{A(\mathsf{sample_i}) = \mathsf{Target_i} \, | \,  H_1 \textrm{ is true}}
\end{aligned}
\end{equation}
%Note that our choice implies that these probabilities are computed on samples such that $\mathsf{True_i} \neq \mathsf{Target_i}$. 
Note that the measure $\hat{r}$ approaches $q$ if the null hypothesis $H_0$ (data was deleted) is true and approaches $p$ if the alternative hypothesis $H_1$ (data was not deleted) is true. To decide whether we are in $H_0$ or $H_1$, we define a threshold $t$ and if $\hat{r} \leq t$ we output $H_0$ else output $H_1$. The false-positive error $\alpha$ (Type I error) and false-negative error $\beta$ (type II error) are the respective leftover probability masses that we have decided wrongly. This is illustrated in \cref{fig:singlesample}.

The threshold $t$ is set according to the desired properties of the hypothesis test. As common in statistics, $t$ is set based on a small value of $\alpha$ (also known as p-value), the probability that we falsely accuse the ML-provider of dismissal of our data deletion request. 

% \subsection{Computing $\ourmetric{A, \alpha}{s,n}$}
\subsection{Estimating Deletion Confidence}
To derive an analytic expression for $\ourmetric{A, \alpha}{s,n}$, we note that the order in which we request the prediction of backdoored samples does not matter.
Moreover, we assume that the ML provider returns the correct target prediction label with probability $q$ for users with fulfilled deletion requests, and $p$ otherwise.
Further, we assume that the ML provider is not aware which user is querying. Else, the provider could run user specific evasion strategies, e.g., having for each user a unique model with only the user's data excluded.
This can, for example, be achieved by an anonymous communication channel. Since the user strategy is completely defined by the the two parameters $q, p$, we will often interchangeably express a strategy $s$ for these cases by $s=(q,p)$.

First, we show that the occurrence probability of a user-measured average backdoor success ratio $\hat{r}$ follows a binomial distribution with abscissa rescaled to [0,1] with mean $q$ (deleted), or $p$ (not deleted) respectively. Then, we compute the Type II error $\beta$ based on the Type I error $\alpha$ that results from the overlap of these two binomial distributions. Finally, we derive an analytic expression for the verification confidence:

\begin{theorem}\label{thm:computerho}
For a given  ML-mechanism $A$ and a given acceptable Type I error probability $\alpha$, the deletion confidence $\rho_{A, \alpha}(s, n)$ is given by the following expression:
\begin{equation}\label{eq:rhoexpression}
\begin{aligned}
    \rho_{A, \alpha}(s, n) &= 1 - \sum_{k=0}^n \binom{n}{k} p^k(1-p)^{n-k} \cdot \\
    &~~~~~~~~~~ \heavyside{\sum_{l = 0}^k \binom{n}{l} q^l(1-q)^{n-l} \leq 1 - \alpha }
\end{aligned}
\end{equation}
where $p,q$ are as given by \cref{eq:pandq} and $H(\cdot)$ is the heavy-side step function, i.e., $H(x) = 1$ if $x$ is $\mathsf{True}$ and $0$ otherwise. 
\end{theorem}

%\grey{Comment by Liwei: the theorem looks like incorrect, the heavy-side step function should be $H(\sum_{l = 0}^k \binom{n}{l} q^l(1-q)^{n-l} \leq 1-\alpha)$}
\Cref{thm:computerho} gives a closed-form expression to compute the backdoor success probability as a function of the various system parameters. To prove the above result, we rely on the independence of prediction order assumption. We define a test of the backdoor success of $n$ consecutive samples as follows: 

\begin{definition}
Given oracle access to the predictions on $n$ samples $\{\mathsf{sample_i}\}_{i=1}^n$, for $r\in[0,1]$, we define $\testacc{n}{r}$ as a random variable that returns a value in $\{0,1\}^n$ where each entry is 1 with probability $r$ and 0 with probability $1-r$ assuming the order of the predictions is immaterial and that they are processed independently.
\end{definition}

If $r$ is set to the backdoor success probability $p$ or $q$, then the above defined $\testacc{n}{r}$ mimics the output of the corresponding ML-mechanism as it effectively measures the ratio of cases where a backdoor was able to change the prediction of its sample to a target label. Hence, for the hypothesis test, it is sufficient to compare the backdoor success ratio $p$ where the backdoor works (data not deleted) to the case where it does not work (data deleted) with ratio $q$. Next, we prove that the random variable $\hat{r}$ follows a rescaled binomial distribution. 

\begin{lemma}[Measured backdoor success rate]\label{lemma:measured}
Let $n \in \mathbb{N}$. Let $o \in \{0,1\}^n$ be a random draw from $\testacc{n}{r}$ with $r\in[0,1]$, the following statements hold: 
% \TODO{the scientific way to write \Pr [ \hat{r} \geq x ] is the summation over the ceil of  n*x to n, similar for equation (8a)}
\begin{enumerate}
    \item The random variable $\hat{r} = \frac{1}{n} \sum_{j=1}^n o_j$ follows a binomial distribution with abscissa scaled to $[0,1]$ with draws $n$ and success probability $r$ where $o_j$ is the $j^{\tiny{\mathrm{th}}}$ draw output of $o$. 
    %In other words, $\Pr[\hat{r} = \frac{i}{n}]$ for $i\in \{0,\ldots,n\}$ follows a binomial distribution with abscissa scaled to $[0,1]$ with draws $n$ and success probability $r$. 
    We call $\hat{r}$ the discrete success rate probability.
    \item The standard-deviation of $\hat{r}$ shrinks as $O(\frac{1}{\sqrt{n}}$)
    \item The tail probability mass of $\hat{r}$ can be computed for $x\in [0,1]$ using the following relation (and a symmetric relation for $\hat{r} \leq x$):
        \begin{equation}\label{eq:tailbounds}
          \Pr [ \hat{r} \geq x ] = \sum_{k \geq  n\cdot x }^n \binom{n}{k} r^k(1-r)^{n-k}
        \end{equation}
\end{enumerate}
\end{lemma}

\begin{proof}
As we assumed the independence of prediction order,
the output of $\testacc{n}{r}$ follows a binomial distribution $\binomdistr{n}{r}$ where $n$ is the number of draws and $r$ is the success probability.
\begin{enumerate}
    \item For $k\in\{0,\ldots,n\}$, let $\mathcal C_k$ be the set of all possible outputs $c$ of $\testacc{n}{r}$ with $\sum_{j=0}^n c_j = k$. Note that all outputs are equally likely. Then, the occurrence probability for $\hat{r} = \frac{k}{n}$ is given by:
        \begin{equation}\label{eq:binomdistr}
        \begin{aligned}
            \Pr[\hat{r} = \frac{k}{n}] 
            &= \sum_{\forall c \in \mathcal C_k} r^k(1-r)^{n-k}\\
            &= \binom{n}{k} r^k(1-r)^{n-k} \\
            &= \Pr_\binomdistrlabel[ k = k | n,r] 
        \end{aligned}
        \end{equation}

    \item The variance of a binomial distribution is $\sigma_n^2 = nr(1-r)$. With scaled abscissa by $1/n$, the standard deviation becomes $\sigma = \sqrt{\sigma^2_n / {n^2}} = {\sqrt{r(1-r)}}/{\sqrt{n}}$.
%$\sigma = \sqrt{\sigma^2} = \sqrt{\frac{\sigma^2_n}{n^2}} = \frac{\sqrt{r(r-1)}}{\sqrt{n}}$.    

    \item The mass in the tail is the sum over the probabilities for the corresponding discrete events. Hence \cref{eq:tailbounds} directly follows from summing \cref{eq:binomdistr} for $k\geq n\cdot x$
\end{enumerate}
\end{proof}

\begin{proof}[Proof of \Cref{thm:computerho}]
\Cref{lemma:measured} can be directly applied to prove the results in \Cref{thm:computerho}. In particular, the hypothesis test consists of distinguishing two scaled binomial distributions with $r=q$ in case $H_0$ (the data has been deleted) and $r=p$ for $H_1$ (data has not been deleted). \Cref{fig:singlesample} graphically illustrates this while \cref{fig:multiplesample} demonstrates the effect of multiple samples on the scaled distributions. As seen in \Cref{lemma:measured}, the scaled distributions concentrate around the mean, thus reducing the probability in the overlapped areas, which in effect reduces the Type I and Type II error probabilities.

By \Cref{lemma:measured}, the shape of the hypothesis distriubtions depens on $q$ for $H_0$ and $p$ for $H_1$. Therefore, for a given a threshold $t \in [0,1]$, the Type I error $\alpha_t$ and the Type II error $\beta_t$ for the hypothesis test depend on $p$ and $q$ respectively.    
\begin{subequations}\label{eq:alphaandbetat}
  \begin{align}
    \begin{split}
            \alpha_q^t &= \Pr[\hat{r} > t | H_0, n ] \\
                        &= \sum_{k >  n\cdot t }^n \binom{n}{k} q^k(1-q)^{n-k}
    \end{split}
    \label{eq:alphat} 
    \\
    \begin{split}
            \beta_p^t  &= \Pr[\hat{r} \leq t | H_1, n] \\
                        &= \sum_{k = 0 }^{n\cdot t} \binom{n}{k} p^k(1-p)^{n-k}
    \end{split}
    \label{eq:betat} 
  \end{align}
\end{subequations}

Given that $\alpha$ is set by systemic constraints, we invert \cref{eq:alphat} to get the optimal value of the threshold $t$ and then plug that into \cref{eq:betat}. 
%In other words, we can determine $t(\alpha)$ given an $\alpha$ and $q$, looking at what $t$ we have a tail smaller than $\alpha$. This is given by:
%\begin{equation}
%    t = \sum_{k=0}^n \frac{1}{n} \heavyside{\Pr\left[\hat{r} \leq \frac{k}{n} \Big|H_0, n\right] \leq 1 - \alpha }
% \end{equation}
Consider the following equality defining $t_\alpha$ given $\alpha$:
\begin{equation}
     \heavyside{\frac{k}{n} \leq t_\alpha} := \heavyside{\Pr\left[\hat{r} \leq \frac{k}{n} \Big|H_0, n\right] \leq 1 - \alpha }
\end{equation}


We can then use this implicit definition of threshold $t_\alpha$ to determine the Type II error $\beta$ given a value of $p$: 
% \TODO{David: Can you please check the ranges of these summations once?} 
% David: summation is correct now. 
\begin{align*}
    \beta_{p,q}^\alpha\! 
    &= \!\sum_{k=0}^n \Pr\left[\hat{r} = \frac{k}{n} \Big| H_1, n\right]\! \cdot \heavyside{\frac{k}{n} \leq t_\alpha} \\
    &=  \!\sum_{k=0}^n \Pr\left[\hat{r} = \frac{k}{n} \Big| H_1, n\right]\! \cdot \heavyside{\Pr\left[\hat{r} \leq \frac{k}{n} \Big|H_0, n\right] \leq 1\! -\! \alpha} \\
     &= \!\sum_{k=0}^n \binom{n}{k} p^k(1\!-\!p)^{n\!-\!k}\! \cdot \heavyside{\sum_{l = 0}^k\!\binom{n}{l} q^l(1\!-\!q)^{n\!-\!l} \leq 1\! -\! \alpha }
\end{align*}
Finally, to connect this value with $\rho_{A, \alpha}(s, n)$, we use \cref{eq:test} from \cref{sec:formulation} and $s=(p,q)$:
\begin{equation}
\begin{aligned}
    \rho_{A, \alpha}(s, n) &= 1- \beta_{p,q}^\alpha \\ 
                           &= 1 - \sum_{k=0}^n \binom{n}{k} p^k(1-p)^{n-k} \cdot \\
    &~~~~~~~~~~ \heavyside{\sum_{l = 0}^k \binom{n}{l} q^l(1-q)^{n-l} \leq 1- \alpha }
\end{aligned}
\end{equation}
which gives us an analytic expression for the confidence that we are in case $H_1$, i.e. that our data has not been deleted as requested. If this value is high, the user has high confidence that the server does not follow deletion request. 
%$H_0$, i.e. that our data has been deleted. If this value is high, the user has high confidence that our data has been deleted. 
%\TODO{the previous version says the confidence is for $H_0$, which I think is reversed. I just change to $H_1$, please check whether I am wrong or not.}
\end{proof}



\subsection{Relaxing Assumptions: Single User Perspective} \label{sec:analysis:bounds}
In our theoretical analysis above, we have assumed to know $p$ and $q$ perfectly. In a real-world setup, these values are always measurements. While a machine learning service provider has the ability to quantify $p$ and $q$ accurately on a lot of samples, single users that want to verify the deletion of their data do usually not have this kind of opportunity. They need to work with vague estimates $\hat{p}$ and $\hat{q}$ obtained on a low number of samples $n$ as described in \cref{sec:oursystem}. 

%To counter the imprecision of $\hat{p}$ and $\hat{q}$ it is sufficient to bounds.
We observe that if we overestimate $\hat{q}$ with a bound  $\hat{q}'$ and underestimate $\hat{p}$ with a bound $\hat{p}'$, then the metric $\rho_{A, \alpha}(s, n)$ provides a lower bound, i.e., the confidence guarantees given by $\rho$ do not worsen if the distance between $\hat{q}$ and $\hat{p}$ increases.
\begin{equation}
\rho_{A, \alpha}(s=(\hat{q}',\hat{p}'), n) \leq \rho_{A, \alpha}(s=(\hat{q},\hat{p}), n) 
\end{equation}
with  $\hat{q} \leq \hat{q}'$ and $\hat{p} \geq \hat{p}'$. This comes from the fact that for a given $\alpha$ the overlap of the two scaled binomial distribution decreases when they are moved further apart, and thereby decreasing the $\beta$ which in terms defines $\rho$.

Alternatively, users can assume priors for $p$ and $q$, apply Bayes' theorem, and compute $\rho_{A,\alpha}$ as the expectation over all possible $p$ and $q$:
\begin{equation}
\Pr[r | \hat{r},n] = \frac{\Pr[\hat{r} | r,n]\,\Pr[r]}{\Pr[\hat{r}|n]}
\end{equation}
for $r\in\{q,p\}$ given an estimation $\hat{r} \in \{\hat{q},\hat{p}\}$. ($\Pr[\hat{r}|n] = \sum_r \Pr[\hat{r} | r,n]$.) Then
\begin{equation*}
\ourmetric{A, \alpha}{s=(\hat{q},\hat{p}),n} = \text{E}_{\Pr[q | \hat{q},n],\Pr[p | \hat{p},n]}\left[\rho_{A, \alpha}(s=(q,p), n)\right]
\end{equation*}


==> Sections/approach.tex <==
\section{Our Framework}\label{sec:oursystem}
% conneciton to problem formulation.

\TODO{Add the ``'interested users'' thing. Emphasize that we don't need everyone to use the system}

\input{Images/system_figure}


Verified machine unlearning is in general very hard given that the data has already been outsourced to another party. Specific to the context of machine-learning-as-a-service (MLaaS), how does one verify if the model is trained on a particular user's data or not? One possible approach is enabled by membership inference attacks such as Shokri et al.~\cite{shokri_membership_SP17} or the approach by Song and Shmatikov~\cite{Mem_song_kdd19}. However, this line of work suffers from a number of limitations -- low accuracy due to the training data not being actively perturbed, extensive knowledge of the MLaaS model's architecture for  white-box attack variants, access to auxiliary or shadow data and computational power in an extent similar to the MLaaS provider -- all of which limit the feasibility of such approaches for our problem setting.
%Instead, our proposed verification framework works by each individual user injecting a user-specific backdoor into the model.

%\TODO{weird structure here, we never mention backdoor as our method, but in threat model, we say the adaptive server uses backdoor defense. Currently, I just add a brief line above to introduce backdoor. also add explanations of not mentioning data erase from hard disk, to prevent the malicious sever benefits by not providing correct prediction, we assume the server cannot distinguish between users. Leave it to david, we should also ask Prateek to read the edits}

\textbf{Threat Model and Assumptions:} We aim to distinguish the scenario of an honest server who follows the data unlearning protocol from that of a dishonest server who can arbitrarily deviate from the protocol. In particular, we consider two specific models for the server in the latter case -- both do not delete the data, but the first is non-adaptive and expects to not get detected, while the second is adaptive and employs state-of-the-art defense mechanisms to mitigate user strategies and to evade detection. 
We run our evaluation on both, adaptive and non-adaptive, server algorithms. \ds{We require that users can control and manipulate the data before they provide it for training. We require only black-box prediction access to the MLaaS provider's model.} However, the provider is not able to determine which user is querying the trained machine learning model. This can be achieved using of-the-shelf anonymous communication schemes like~\cite{tor,vuvuzela}. Finally, we note that the scope of our approach is limited to validating if users' data was deleted from a specific machine learning model exposed by the MLaaS provider, and does \emph{not} include validating deletion from other computing or storage resources at the provider.   
%The MLaaS provider knows the correspondence between user and the corresponding submitted training data, but we assume that it is not possible to determine who queries the trained machine learning model. This can be achieved using of-the-shelf anonymous communication schemes like~\cite{tor,vuvuzela}. 
%For the determination of the confidence of the hypothesis test, we assume that the predicted labels are independent of each other and that the predicting order does not matter.

\textbf{Our Approach: }\red{David: the rest of this section needs some rewriting} In order to enable such a system for verifying machine unlearning, we propose an approach that leverages the users' ability to inject stealthy backdoors into their data. In particular, \ds{privacy enthusiasts modify} their data locally using a \textit{private backdoor} that is only known to them individually. If the MLaaS provider trains the model on such data, the backdoor can help the user detect maliciously dismissed data deletion requests as the models trained on the \textit{poisoned data} (the data which contains such private backdoors) provide different predictions on very specific samples compared to models trained on data without poisoning. Compared to prior work on backdoors (cf. \cref{sec:background}), we  propose and analyze a multi-user scenario where each user \ds{can employ} an individual backdoor.
 
For such a system to work well, it is imperative that there exists a statistically significant distinguishing test between models trained \textit{with} vs \textit{without} the backdoored user's data. At the same time, the backdoored data should have minimal impact on the model's normal performance. %These two opposing objectives make it hard to design systems that provide both these requirements. 
\Cref{fig:system_design} shows our approach and can be described in two phases as follows:\\

\noindent \textbf{Phase I}
\begin{enumerate}
    \item The users generate individual backdoor patterns that alter the predictions of samples to a fixed label. 
    %(cf \cref{sec:collisions} for an analysis of similar backdoors by different users).
    \item Users apply their backdoor patterns to a fraction of their data, submit that to the MLaaS provider, and the provider trains a ML model on the data.
    \item Each user can run confirmation tests to collect statistics on their backdoor.
\end{enumerate}

\noindent \textbf{Phase II}
\begin{enumerate}
    \item Some users request a deletion of their data. The server then either retrains the model complying with these requests or proceeds maliciously.
    \item The users query model with $n$ backdoored samples and based on the predictions try to infer if the server complied with their request or not.
\end{enumerate}

% Our approach does not require detailed understanding of MLaaS provider's computation. Instead, each client augments its individual data with a random individual backdoor that alters the prediction behaviour of the provider's ML algorithm if the provider uses the data for training. Then the client submit the data to the provider to be used in training. To determine whether the data has been used for training after a deletion request, the client queries the trained model and checks whether testing samples with its individual backdoor applied are able to alter the prediction of the provider's model. For simplicity, this work only considers classification tasks but the proposed approach is not limited to these. %illustrates the proposed process. 
% \grey{Comment by Liwei: we may need to rephrase the description here -- to enable user to determine whether its data was used to train the model, we need to embed some ``watermarks/traces/taints/tagging'' into the training set such that ML models trained on it can be identified easily. At the same time, such ``traces/tagging'' should have little or no impact on ML models' normal performance.
% Backdoor satisfies the above two requirements! Then describe what is backdoor using \Cref{fig:system_design}}

%\TODO{the following paragraphs are not well-written, maybe ask Prateek for sanity check!}

In our evaluation (\cref{sec:evaluation}), we apply a backdoor using the method described in \cref{sec:background:backdoormethod}, i.e, setting 4 user-specific pixel or words to a dataset dependent value and changing the label to a user-specific target label. 
Note that the success of altering the prediction using backdoored samples is usually not guaranteed every single time but in a probabilistic manner. Thus, the decision on whether the data has been deleted or not is determined by a hypothesis test. For an effective backdoor algorithm, when the model was trained on backdoored data, the probability of receiving the target label in presence of the backdoor pattern, i.e., backdoor success rate, should be high. At the same time, when the provider has deleted the user's data (the model has not been trained on the user's backdoored samples), the backdoor success rate should be low. 
In this way the hypothesis test can distinguish between the two scenarios. Throughout this paper, the two probabilities corresponding to backdoor attack accuracy for deleted data and undeleted data are referred to as $q$ (lower), and $p$ (higher) respectively. 
Furthermore, the confidence of this test increases with $n$, the number of backdoored test samples a user queries the trained ML model with.
Thus our verification mechanism can be used to detect missing deletion with high confidence by increasing the number of test samples. 
%Thus, the backdoor technique applied needs to have a success probability that differs from the random prediction baseline. The more they differ, the fewer testing queries are needed to determine whether the data has been deleted or not. 

Given that estimation of $p$ and $q$ is central to the detection of non-compliance, we describe the approach from an individual user perspective below.

\textit{Estimating $p$:} A user can obtain an estimate $\hat{p}$ by querying the model with backdoored samples, immediately after the model has been trained with its data. At this moment, a user can determine whether the backdoor strategy is working. If the resulting $\hat{p}$ is close to the random prediction  baseline, either the applied backdoor strategy $s$ is not working, or its data has not been used in training. However, if $\hat{p}$ is significantly higher than the baseline, our strategy $s$ can work well %was successful
and we can use $\hat{p}$ as an estimate.

\textit{Estimating $q$:} There are two ways of obtaining an estimate $\hat{q}$: If the algorithm can be queried before the user provides its data, $\hat{q}$ can be obtained by querying the algorithm using samples with the user's backdoor the algorithm has not seen before. If this is not possible, the user can estimate $\hat{q}$ by applying another random backdoor pattern to its data and querying the algorithm. The output should be similar to the case where the algorithm has never seen the user's legitimate backdoor pattern. 



%%%%%% stepwise detailed explanation
% In detail, our approach illustrated in \Cref{fig:system_design} works as follows:
% \begin{enumerate}
%     \item Client generates an individual backdoor than alters predictions to a fixed label. Due to the high number of possibilities, we neglect collisions. 
%     \item Client applies backdoor to a fraction of its data.
%     \item Clients give their data to the MLaaS provider.  
%     \item Provider trains ML algorithm.
%     \item \grey{Client test for their $\hat{p}$.}
%     \item Client requests deletion.
%     \item After the provider announced re-generation of the model, client queries model with $n$ backdoored samples and saves predictions. 
%     \item Client determines with received predictions an estimate of the backdoor success probability $\hat{m}$.
%     \item Client confirms or objects provider's deletion statement with desired confidence. 
% \end{enumerate}

==> Sections/formulation.tex <==
\section{Problem Formulation}\label{sec:formulation}

{\color{magenta} Sameer take a pass at this!!.}


\TODO{Add the ``'interested users'' thing. Emphasize that we don't need everyone to use the system. What is old and what is new? Add that users can control what data they submitt, but they cannot control what is used and hat is stored by the ML provider. We should define the term poison ratio}
%\input{Images/general}

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cll} 
\toprule
Symbol          & Range                     & Description \\
\midrule
$n$             & $\mathbb{N}$      	 	& Number of test service requests\\
$\alpha, \beta$ & $[0,1]$                   & Type I, II errors (cf Eq.~\ref{eq:beta})\\
$p, q$          & $[0,1]$                   & Probabilities for analysis (cf Eq.~\ref{eq:pandq})\\
\mr{2}{$f_{\mathsf{user}}$}             & \mr{2}{$[0,1]$}                   & Fraction of users that are privacy enthusiasts \\
& &                                                                         (i.e., those who are verifying \ds{unlearning}) \\
\mr{2}{\ds{$f_{\mathsf{data}}$}}        & \mr{2}{$0$-$100\%$}               & Percentage of data samples poisoned by \\
 & &                                                                          each privacy enthusiast\\
\mr{2}{$\ourmetric{A, \alpha}{s, n}$} & \mr{2}{$[0,1]$}     & Effectiveness of a verification strategy $s$, a model \\
                &                            & training algorithm A and acceptable Type I error $\alpha$\\
%                &                           & Anything else?\\
\bottomrule 
\end{tabular}
}
\caption{Notation used in this work. \red{Reference this.}}
\label{table:notation}
\end{table}



%In this section, we formalize a theoretical framework that will enable the study of a large class of backdoors and defenses \grey{the formulation is quite general, not limited to backdoors, right?} in the context described in Section~\ref{sec:datadeletionverification}. 
In this section, we formalize a framework to study machine unlearning in the context of MLaaS. Specifically, we consider the following scenario illustrated in \Cref{fig:system_train}: Users interact with a server who provides machine learning as a service. Users who request the removal of their data from the training set of a machine learning service have no guarantee currently that their data was actually removed. 
Thus, there is an important need to uncover a strategy that can verify if user data was used in the generation of a machine learning model\footnote{Note that given the difficult of verifying local computations on the server, % side, 
it is difficult to infer \textit{directly} if the data was used in the training set or not.}. We formalize a framework to study the effectiveness of such machine unlearning verification strategies.
%They would like to employ a strategy that can detect if their data was used in the generation of the machine learning model
 
\sw{To study the effectiveness of any strategy employed by the users, we use a standard hypothesis test~\cite{}. This has been well studied in the statistics literature and forms a rigorous foundation for our framework. Next we lay the groundwork to describe the hypothesis test for our problem. Note that in Section~\ref{sec:analysis}, we provide the required calculations to give a closed form expression for the effectiveness of our strategies as well as study other important characteristics such as the effectiveness of the strategy given that the users do not know the ground truth parameters.} 
 

\paragraph{Notation} \red{REMOVE THIS.} Let $\calU$ denote the set of all users and $u \in \calU$ denote a particular user. Let $s \in \calS$ denote a specific strategy used by the users to verify whether the server deletes its data following the deletion request\footnote{We restrict our analysis to a single strategy, with local randomness, used by all the users.} where $\calS$ denotes the space of all possible users strategies. Furthermore, let $A \in \calA$ denote the model training algorithm used by the server where $\calA$ denotes the set of all possible algorithms that can be used by the server. For generality, we consider that such a service allows for multiple requests. We assume that the users use MLaaS while injecting a few \textit{test service requests} (denoted by $n$) which will be used to detect server malintent. We then formulate the effectiveness of such machine unlearning verification strategies using %standard statistics 
hypothesis testing.
%To this end, we assume the servers inability to distinguish benign service requests from test service requests. Note that such an assumption can be easily justified through the use of anonymous communication channels~\cite{tor}. In particular, let $n$ denote the number of test service requests sent by the user. Let $A = A_0$ denote a server strategy that follows the protocol i.e., it deletes the user data and generates the model accordingly. We formulate the effectiveness of such strategies using standard statistics hypothesis testing.

% \paragraph{Indistinguishability Game.} We consider the following indistinguishability game played between the user and the server. 

\paragraph{Hypothesis Testing} We define the \textit{null hypothesis} $H_0$ to be the state when server deletes the user data and the \textit{alternative hypothesis} $H_1$ to be the state when the server does not delete the data.
%\red{comment by Liwei: this part is confusing, we mention $A = A_0$ for $H_0$, here it should be $A = A_{1}$ where the server does not delete the data, right? Also, do we really need the notation $A$?}
We define the Type I errors as  $\alpha$ (false positive) and Type II errors as $\beta$ (false negative) given below:
\begin{equation}
\begin{aligned}
  \alpha &= \pr{\textrm{Reject } H_0\, |\, H_0 \textrm{ is true}} \\
  \beta &= \pr{\textrm{Accept } H_0\, |\, H_1 \textrm{ is true}}\label{eq:beta}
\end{aligned}
\end{equation}

%\red{David: actually in sloppy terms, rho is the deletion confidence}
We define the effectiveness of a verification strategy $s$ for a given server algorithm $A$ for a given acceptable tolerance of Type I error ($\alpha$) to be the power of the hypothesis test formulated above, i.e.,
\begin{equation}\label{eq:test}
\begin{aligned}
    \ourmetric{A, \alpha}{s, n} &= (1-\beta) \\ 
    &= 1 - \pr{\textrm{Accept } H_0 | H_1 \textrm{is true}}
\end{aligned}
\end{equation}

Informally speaking, $\rho$ quantifies the confidence the user has that the server has deleted their data. This deletion confidence $(1-\beta)$, the power of the hypothesis test, is the probability that we detect the alternative hypothesis when the alternative hypothesis is true. On the other hand, $\alpha$ refers to the acceptable value of the server being falsely accused of malicious activity when in practice it follows the data deletion honestly. For a given value of $n$,  $\alpha$ and $\beta$ cannot be simultaneously reduced and hence we usually set an acceptable value of $\alpha$ and then $(1-\beta)$ quantifies the effectiveness of the test.

%Users who want their data deleted from the training set of a machine learning service have no guarantee currently that their data was actually deleted. 

%We try to quantify how well does a backdoor algorithm $B$ works in providing a solution for the problem of the ``right to be forgotten''. This is a function of the server algorithm as well as ...

% $s \in S$ is the user strategy and $A$ is a given server behaviour

% Then we want to quantify 

% \begin{equation}
%     \rho_{A,p}(S = s, N = n) = p (detection(s, A) - detection(s, A_b))
% \end{equation}

% $A_b \rightarrow$ deletes data 

% background work: Naive solution 1: $s = $ membership inference and show that it doesn't work well? 
% Better solution: Use our backdoor 

==> Sections/new_formulation.tex <==
\section{Formal Testing of Machine Unlearning}\label{sec:formulation}

In this section, we formalize a framework to study machine unlearning in the context of MLaaS. Specifically, we consider the following scenario illustrated in \Cref{fig:system_train}: Users interact with a server who provides machine learning as a service (MLaaS). Users who request the removal of their data from the training set of a machine learning service have no guarantee currently that their data was actually removed. They would like to employ a strategy that can detect if their data was used in the generation of the machine learning model\footnote{Note that given the difficult of verifying local computation on the server side, it is difficult to infer directly if the data was used in the training set or not.}. We formalize a framework to study the effectiveness of such strategies. 

\subsection{Problem Definition}
Let $\calU$ denote the set of all users and $u \in \calU$ denote a particular user. Let $s \in \calS$ denote a specific strategy used by the users\footnote{We restrict our analysis to a single strategy, with local randomness, used by all the users.} where $\calS$ denotes the space of all possible users strategies. Furthermore, let $A \in \calA$ denote the algorithm used by the server where $\calA$ denotes the set of all possible algorithms that can be used by the server. For generality, we consider that such a service is running allows for multiple requests. We assume that the users use MLaaS while injecting a few \textit{test service requests} (denoted by $n$) which will be used to detect server malintent. We then formulate the effectiveness of such strategies using standard statistics hypothesis testing.

\paragraph{Hypothesis Testing.} We define the \textit{null hypothesis} $H_0$ to be the state when server deletes the user data and the \textit{alternative hypothesis} $H_1$ to be the state when the server does not delete the data. We define the Type I errors as  $\alpha$ and Type II errors as $\beta$ given below:
\begin{equation}
\begin{aligned}
  \alpha &= \pr{\textrm{Reject } H_0\, |\, H_0 \textrm{ is true}} \\
  \beta &= \pr{\textrm{Accept } H_0\, |\, H_1 \textrm{ is true}}\label{eq:beta}
\end{aligned}
\end{equation}

We define the effectiveness of a strategy $s$ for a given server strategy $A$ for a given acceptable tolerance of Type I error ($\alpha$) to be the power of the hypothesis test formulated above i.e.,
\begin{equation}\label{eq:test}
\begin{aligned}
    \ourmetric{A, \alpha}{s, n} &= (1-\beta) \\ 
    &= 1 - \pr{\textrm{Accept } H_0 \, | \, H_1 \textrm{is true}}
\end{aligned}
\end{equation}

Informally speaking, $\rho$ quantifies the confidence the user has that the server has deleted their data. $(1-\beta)$ or the power of the hypothesis test is the probability that we accept the alternative hypothesis when the alternative hypothesis is true. On the other hand, $\alpha$ refers to the acceptable value of the server being falsely accused of malicious activity when in practice it follows the data deletion honestly. For a given value of $n$,  $\alpha$ and $\beta$ cannot be simultaneously reduced and hence we usually set a low value of $\alpha$ and then $\beta$ quantifies the effectiveness of the test.


\subsection{Our Approach: Using Backdoor Algorithms}

\input{Images/system_figure}

Verified deletion of data is in general very hard given that the data has already been outsourced to another party. Specific to the context of machine-learning-as-a-service (MLaaS), how does one verify if the model is trained on a particular user's data or not? One possible approach is enabled by membership inference attacks such as Shokri et al.~\cite{shokri_membership_SP17} or those proposed in Song and Shmatikov~\cite{Mem_song_kdd19}. However, this line of work suffers from a number of limitations -- low accuracy, strong assumptions on the users, and a passive detection method -- all of which limit the feasibility of such approaches for our problem setting.

\textbf{Threat Model and Assumptions: }We assume a dishonest server who either follows the protocol (deletes the user data) or can arbitrarily deviate from the protocol. In particular, we consider two specific models for the server in the latter case -- the first does not delete the user data and expects to not get detected and the second which employs state-of-the-art backdoor defense mechanisms to evade detection. We run our evaluation on both these server algorithms. Our approach requires only black-box prediction access to the MLaaS provider's model. For the determination of the confidence of the hypothesis test, we assume that the predicted labels are independent of each other and that the predicting order does not matter.

\textbf{Our Backdoor Algorithm: }In order to enable such a system, we look at an approach that leverages the users' ability to inject stealthy backdoors into their data. In particular, each user modifies their data locally using a \textit{private backdoor} that is only known to them. If the MLaaS provider trains the model on such data, the backdoor can help the user detect such behaviour as the models trained on the \textit{poisoned data} (the data which contains such private backdoors) provide different predictions on very specific samples compared to models trained on data without poisoning. 
 
For such a system to work well, it is imperative that there exists a statistically significant distinguishing test between models trained \textit{with} vs \textit{without} the backdoored user's data. At the same time, the backdoored data should have little or no impact on the ML model's normal performance. These two opposing objectives make it hard to design systems that provide both these requirements. \Cref{fig:system_train} shows our approach and can be described in two phases as follows:\\

\noindent \textbf{Phase I}
\begin{enumerate}
    \item The users generate individual backdoors that alter the predictions of samples to a fixed label (cf \cref{sec:collisions} for an analysis of similar backdoors by different users).
    \item Users apply their backdoors to a fraction of its data, submit that to the MLaaS provider and the provider runs the ML service on the data.
    \item Each user can run preliminary tests to collect statistics on their backdoor.
\end{enumerate}

\noindent \textbf{Phase II}
\begin{enumerate}
    \item Some users request a deletion of their data, the server then either retrains the model complying with these requests or proceeds maliciously.
    \item The users queries model with $n$ backdoored samples and based on the predictions try to infer if the server complied with their request or not.
\end{enumerate}

Note that the success of altering the prediction using backdoored samples is usually not guaranteed every single time but in a probabilistic manner. Thus, the decision whether the data has been deleted or not is determined by a hypothesis test. For a good backdoor algorithm, when the model has been trained on backdoored data, the probability of receiving the poisoned label should be high. At the same time, when the provider has deleted the data and the model has not been trained on the backdoored samples, the probability of receiving the poisoned label should be low. In this way the hypothesis test can distinguish between the two scenarios. Throughout this publication, the two probabilities are referred to as $q$ for the lower, and $p$ for the higher one respectively. Furthermore, the confidence of this test increases with $n$, the number of test samples and hence such an approach can be used to distinguish with high confidence. 



\subsection{Single User Perspective}
For a given backdoor technique, it is desirable to have a success probability that differs from the random prediction baseline. The more they differ, the fewer testing queries are needed to determine whether the data has been deleted or not. Given that estimation of $p$ and $q$ is central to the detection, we briefly describe the approach from an individual user perspective below since these values can not be directly computed by individual users.

\textit{Estimating $p$:} A use can obtain an estimate $\hat{p}$ by querying the model with backdoored samples, immediately after the model has been trained with its data. At this moment, a user can determine whether the backdooring strategy is working. If the resulting $\hat{p}$ is close to the \grey{(specify which)} baseline, either the applied strategy $s$ is not working, or its data has not been used in training. However, if $\hat{p}$ is significantly higher than the baseline, our strategy $s$ was successful and we can use $\hat{p}$ as an estimate.

\textit{Estimating $q$:} This is more tricky as $\hat{p}$ because the user assumes its data has been used by the algorithm. There are two ways of obtaining an estimate $\hat{q}$: Either if the algorithm can be queried before the user provides its data, $\hat{q}$ can be obtained by querying the algorithm using samples with the user's backdoor the algorithm has not seen before. Or, if this is not possible, the user can estimate $\hat{q}$ by apply another random backdoor pattern to its data and query the algorithm. The output should be similar to the case where the algorithm has never seen the users legitimate backdoor pattern. 



==> Tables/dataset_summary.tex <==

\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c c c c c | c c c | c c c c}
\toprule
\multicolumn{5}{c}{\textbf{Dataset Details}} & \multicolumn{3}{c}{\textbf{ML Model}} & \multicolumn{4}{c}{\textbf{Verification Performance (30\% backdooring ratio)}} \\
\multirow{2}{*}{Name} & sample & number of & number of  & number of  & model  & train acc. & test acc. & backdoor  & attack acc.  & attack acc. & $\rho$ $(n=10,$ \\
 & dimension & classes &total samples & total users &  architecture & (no backdoor) & (no backdoor) &  method &  (undeleted users) &  (deleted users) & $\alpha=10^{-3}$) \\
\midrule
\multirow{2}{*}{EMNIST} & \multirow{2}{*}{$28 \times 28$} & \multirow{2}{*}{10} & \multirow{2}{*}{280,000} & \multirow{2}{*}{1,000} & \multirow{2}{*}{MLP} & \multirow{2}{*}{$99.84\%$} & \multirow{2}{*}{$98.99\%$} & set 4 random  & \multirow{2}{*}{$93.64\%$} & \multirow{2}{*}{$9.56\%$} & \multirow{2}{*}{$1-2.0\times10^{-4}$} \\
 & &  &  & & & & & pixels to be 1 & & & \\
\midrule
\multirow{2}{*}{F-EMNIST} & \multirow{2}{*}{$28 \times 28$} & \multirow{2}{*}{10} & \multirow{2}{*}{382,705} & \multirow{2}{*}{3,383} & \multirow{2}{*}{CNN} & \multirow{2}{*}{$99.72\%$} & \multirow{2}{*}{$99.45\%$} & set 4 random & \multirow{2}{*}{$99.98\%$} & \multirow{2}{*}{$10.30\%$} & \multirow{2}{*}{$1-2.7\times10^{-17}$} \\
 & &  &  & & & & & pixels to be 0 & & & \\
\midrule
\multirow{2}{*}{CIFAR10} & \multirow{2}{*}{$32 \times 32 \times 3$} & \multirow{2}{*}{10} & \multirow{2}{*}{60,000} & \multirow{2}{*}{500} & \multirow{2}{*}{ResNet} & \multirow{2}{*}{$98.98\%$} & \multirow{2}{*}{$91.03\%$} & set 4 random & \multirow{2}{*}{$96.93\%$} & \multirow{2}{*}{$8.43\%$} & \multirow{2}{*}{$1-1.6\times10^{-7}$} \\
 & &  &  & & & & & pixels to be 1 & & & \\
\midrule
\multirow{2}{*}{AG News} & \multirow{2}{*}{15--150 words} & \multirow{2}{*}{4} & \multirow{2}{*}{549,714} & \multirow{2}{*}{580} & \multirow{2}{*}{LSTM} & \multirow{2}{*}{$96.87\%$} & \multirow{2}{*}{$91.03\%$} & replace 4 out of & \multirow{2}{*}{$99.95\%$} & \multirow{2}{*}{$26.68\%$} & \multirow{2}{*}{$1-1.5\times10^{-8}$} \\
& &  &  & & & & & last 15 words & & & \\
\bottomrule
\end{tabular}}
\caption{Table to summarize dataset details, model performance, and our key verification results. \TODO{Liwei, I moved the caption to the bottom. Also, I've fixed the compile bug other table}.}
\label{tab:dataset_summary}
\end{table*}

==> Tables/table_edited.tex <==

\begin{table*}
\caption{Table to summarize dataset details, model performance, and our key verification results.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c c c c c | c c c }
\toprule
\multicolumn{5}{c}{\textbf{Dataset Details}} & \multicolumn{3}{c}{\textbf{ML Model}}  \\
\multirow{2}{*}{Name} & sample & number of & number of  & number of  & model  & train acc. & test acc. \\
 & dimension & classes &total samples & total users &  architecture & (no backdoor) & (no backdoor) \\
\midrule
\multirow{2}{*}{EMNIST} & \multirow{2}{*}{$28 \times 28$} & \multirow{2}{*}{10} & \multirow{2}{*}{280,000} & \multirow{2}{*}{1,000} & \multirow{2}{*}{MLP} & \multirow{2}{*}{$99.84\%$} & \multirow{2}{*}{$98.99\%$} \\
 & &  &  & & & & \\
\midrule
\multirow{2}{*}{F-EMNIST} & \multirow{2}{*}{$28 \times 28$} & \multirow{2}{*}{10} & \multirow{2}{*}{382,705} & \multirow{2}{*}{3,383} & \multirow{2}{*}{CNN} & \multirow{2}{*}{$99.72\%$} & \multirow{2}{*}{$99.45\%$} \\
 & &  &  & & & & \\
\midrule
\multirow{2}{*}{CIFAR10} & \multirow{2}{*}{$32 \times 32 \times 3$} & \multirow{2}{*}{10} & \multirow{2}{*}{60,000} & \multirow{2}{*}{500} & \multirow{2}{*}{ResNet} & \multirow{2}{*}{$98.98\%$} & \multirow{2}{*}{$91.03\%$}  \\
 & &  &  & & & & \\
\midrule
\multirow{2}{*}{AG News} & \multirow{2}{*}{15--150 words} & \multirow{2}{*}{4} & \multirow{2}{*}{549,714} & \multirow{2}{*}{580} & \multirow{2}{*}{LSTM} & \multirow{2}{*}{$96.87\%$} & \multirow{2}{*}{$91.03\%$}  \\
& &  &  & & & & \\
\bottomrule
\end{tabular}}
\label{tab:todo}
\end{table*}
